Constrained Optimisation of Rational Functions for Accelerating Subspace Iteration

Earlier this decade, the so-called FEAST algorithm was released for computing the eigenvalues of a matrix in a given interval. Previously, rational filter functions have been examined as a parameter of FEAST. In this thesis, we expand on existing work with the following contributions: (i) Obtaining well-performing rational filter functions via standard minimisation algorithms, (ii) Obtaining constrained rational filter functions efficiently, and (iii) Improving existing rational filter functions algorithmically. Using our new rational filter functions, FEAST requires up to one quarter fewer iterations on average compared to state-of-art rational filter functions.

==> figures/experiments/squared_intergrals.tex <==
\begin{table}
	\centering			
	\pgfplotstabletypeset[
	columns={G,q,gauss,bfgsgamma,ebfgs},
	columns/G/.style={
		precision=6,
		column name=Gap $G$,
	},
	columns/q/.style={
		int detect,
		column name={Poles},
		preproc/expr={4*##1}
	},		
	columns/{gauss}/.style={
		sci,sci zerofill,precision=2,sci superscript,
		column name={\textsc{Gauss-Legendre}}
	},
	columns/{bfgsgamma}/.style={
		sci,sci zerofill,precision=2,sci superscript,
		column name={$\gamma$-\LSOP/} % \makecell{Line 1\\Line 2}
	},
	columns/{box}/.style={
		sci,sci zerofill,precision=2,sci superscript,
		column name={\LBFGSB{}}
	},
	columns/{zolo}/.style={
		sci,sci zerofill,precision=2,sci superscript,
		column name={Elliptic}
	},
	columns/{zolo2}/.style={
		sci,sci zerofill,precision=2,sci superscript,
		column name={Ell. Filter}
	},
	columns/{ebfgs}/.style={
		sci,sci zerofill,precision=2,sci superscript,
		column name={Enhanced $\gamma$-\LSOP/}
	},
	every row no 3/.style={after row=\midrule},
	every row no 7/.style={after row=\midrule},
	every row no 11/.style={after row=\midrule},
	every row no 15/.style={after row=\midrule},
	every row no 19/.style={after row=\midrule},
	every head row/.style={before row=\toprule,after row=\midrule},
	every last row/.style={after row=\bottomrule},
	col sep=comma
	] %
	{figures/experiments/squared_intergrals.dat}
	
	\caption[Squared integrals]{\ACID{} for different \RFF{}s. (smaller is better)}
	\label{tab:squared_intergrals}
\end{table}

==> figures/lossfunction/weightfunction.tex <==
\begin{figure}
	\centering			
	\tikzsetnextfilename{weightfunction}
	\begin{tikzpicture}
	\begin{axis}[
	%enlargelimits=false,
	xmin=-1.5,
	xmax=1.5,
	%restrict x to domain=-2:2,
	%axis y line*=left,
	%axis x line*=bottom,
	xlabel={$x$}, ylabel={$\mathfrak{G}_{\eta\text{-\LSOP/}}(x)$},
	width=1\textwidth,
	height=0.24\textheight,
	%axis background/.style={fill=black!3},
	%tick align=outside,
	]
	\addplot[color=GAUSSC, thick] table[x index={0},y index={1}] {figures/costfunction/weightfunction.dat};
	\end{axis}
	\end{tikzpicture}
	\caption[Simple weight function]{$\eta$-\LSOP/, a simple weight function, as per Example~\ref{exmpl:slise}.}
	\label{fig:weightfunction}
\end{figure}
